A Provably Efficient Model-Free Posterior Sampling Method for Episodic Reinforcement Learning

Thompson Sampling is one of the most effective methods for contextual bandits and has been generalized to posterior sampling for certain MDP settings. However, existing posterior sampling methods for reinforcement learning are limited by being model-based or lack worst-case theoretical guarantees beyond linear MDPs. This paper proposes a new model-free formulation of posterior sampling that applies to more general episodic reinforcement learning problems with theoretical guarantees. We introduce novel proof techniques to show that under suitable conditions, the worst-case regret of our posterior sampling method matches the best known results of optimization based methods. In the linear MDP setting with dimension, the regret of our algorithm scales linearly with the dimension as compared to a quadratic dependence of the existing posterior sampling-based exploration algorithms.

==> apppendix/proofs-notations-backup.tex <==

\appendix

\section{Proof of Theorem~\ref{thm:regret}}

Let
\begin{align}
\label{eqn:Qdef}
\hat{Q}_t^h(\theta)=& 
- (1-\alpha)  \ln p_0^h(\theta^h)
- \alpha \sum_{s=1}^{t-1}
\eta 
\ln \tilde{p}(\theta^h|\theta^{h+1},S_{t-1}) \\
=& 
- \ln p_0^h(\theta^h)
+ \alpha \eta \sum_{s=1}^{t-1}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s)\nonumber\\
&\qquad - \alpha \ln \rE_{\tilde{\theta}^h \sim p_0^h(\theta^h)}
\exp 
\bigg(-
\sum_{s=1}^{t-1}\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s\bigg)
 ,
\nonumber
\end{align}
.
 At episode $t$, we define the conditional posterior sampling probability as of $\theta=[\theta_1,\ldots,\theta_H]$:
 \begin{align}
 \tilde{p}(\theta^h|\theta^{h+1},S_{t-1}) =& \frac{p_0^h(\theta^h)  
 \exp(-\sum_{s=1}^{t-1} L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))}
 {\rE_{\tilde{\theta}^h \sim p_0^h(\cdot)}
 \exp\Bigg(-
 \sum_{s=1}^{t-1}L^h([\tilde{\theta}_t^h,\theta_t^{h+1}],x_s,a_s,r_s)
 \Bigg)
 } \nonumber \\
 \tilde{p}(\theta|S_{t-1})
 =& \prod_{h=1}^H 
 \tilde{p}(\theta^h|\theta^{h+1},S_{t-1}) 
\label{eq:conditional-posterior}
 \end{align}
Note that although $\tilde p(\theta | S_{t-1})$ takes the form of a product of conditional expectations and the optimism term in $p(\theta | S_{t-1})$ only applies to $\theta^1$, the final distribution $p(\theta | S_{t-1})$ the conditional distributions $p(\theta^h | \theta^{h+1}, S_{t-1})$ do not match $\tilde p(\theta^h | \theta^{h+1}, S_{t-1})$. The optimism term biases each conditional expectation.
 Note that this definition is equivalent to
 \[
 \tilde{p}(\theta^{h}_t | \theta_t^{h+1}, S_{t-1})
 \propto
 p_0^h(\theta^{h}_t) \exp\Bigg( 
 - \eta\sum_{s=1}^{t-1} (f^h(\theta^h_t, x_s^h, a_s^h) - r_s^h - f^{h+1}(\theta_t^{h+1}, x_s^{h+1}))^2\Bigg) ,
 \]
 and then define the posterior sampling distribution at time $t$ as follows: \begin{equation}
 \hat{p}_t(\theta_t)
 \propto
 \exp\Bigg(
 (1-\alpha)\sum_{h=1}^H \ln p_0^h(\theta_t^h)+
 \alpha \sum_{h=1}^H \ln \tilde{p}(\theta_t^h|\theta_{t}^{h+1},S_{t-1}) 
 + \lambda f^1(\theta^1_t,x_t^1)
 \Bigg) ,
 \label{eq:conditional-posterior-comp}
 \end{equation}
 or more generally,
 \begin{equation}
 \hat{p}_t(\theta_t)
 \propto
 \exp\Bigg(
 (1-\alpha)\sum_{h=1}^H \ln p_0^h(\theta_t^h)+
 \alpha \sum_{h=1}^H \ln \tilde{p}(\theta_t^h|\theta_{t}^{h+1},S_{t-1}) + \lambda_t \rE_{x_t \sim \hat{D}_t} f^1(\theta^1_t,x_t^1)
 \Bigg) ,
 \label{eq:conditional-posterior-comp-2}
 \end{equation}
 where in \eqref{eq:conditional-posterior-comp-2} we assume that $D_t$ is the distribution of $x_t$, and $\hat{D}_t$ is a random estimation of $D_t$ so that
 \[
 \rE_{\hat{D}_t} \;
 \rE_{x_t \sim \hat{D}_t}
 f^1(\theta,x_t)  = \rE_{x_t \sim D_t} f^1(\theta,x_t) .
 \]
 For example, we may know the distribution of $D_t$, and take $\hat{D}_t=D_t$, or if all $x_t$ comes from the same distribution $D_t=D$, then we may take
 \[
 \rE_{x_t \sim \hat{D}_t}
 f^1(\theta,x_t)
= \sum_{s=1}^{t-1} \lambda_{t,s} f^1(\theta,x_s) ,
 \]
 with $\sum_{s=1}^{t-1} \lambda_{t,s} = \lambda_t$.
 
  Given $\theta_t$ from the posterior, the Thompson Sampling method employs the associated greedy policy $\pi(\theta_t)$ as: at step $h$ and state $x^h$, we pick an action that maximizes the value according to the model
 \begin{equation}
 \pi(\theta_t): \qquad a^h = a^h(\theta_t^h,x^h) . \label{eq:rl-greedy-policy}
 \end{equation}
 This policy induces a distribution on $[x_t,a_t,r_t]$, which we denote as 
 \[
 p(\cdot|\theta_t) :  \quad \text{distribution induced by $\pi(\theta_t)$} .
 \]
 The conditional Thompson Sampling algorithm for reinforcement learning is given in Algorithm~\ref{alg:ts-rl}.
 


\subsection*{Notations}
 


 For notation convenience, we also define the following symbols, which will be used throughout the regret analysis.
 \begin{align*}
  \bar{f}^{h+1}(\theta^{h+1},x^h,a^h)=&\rE_{x^{h+1}|x^h,a^h} 
    f^{h+1}(\theta^{h+1},x^{h+1})\\
 \bar{f}^{h+1}_*(x^h,a^h)=&\rE_{x^{h+1}|x^h,a^h} 
    f^{h+1}_*(x^{h+1})\\
\Delta f^h(\theta^h,x^h,a^h) =& f^h(\theta^h,x^h,a^h)-f_*^h(x^h,a^h) ,\\
\Delta \bar{f}^{h+1}(\theta^{h+1},x^h,a^h) =& \bar{f}^{h+1}(\theta^{h+1},x^h,a^h)-\bar{f}_*^{h+1}(x^h,a^h)   \\
\Delta f^h(\theta^h,x^h) =& f^h(\theta^h,x^h,a^h)-f_*^h(x^h).
 \end{align*}
  
%For simplicity, we consider finite function families with $N_h$ functions at each stage $h$ ($h=1,\ldots,H$), and let $p_0^h(\cdot)$ be the uniform prior on these $N_h$ functions. 

\begin{definition}
We assume that for all $\alpha \in (0,1]$, and  $\epsilon>0$:
\[
\kappa^h(\alpha,\epsilon)=
 (1-\alpha) \ln \rE_{\theta^{h+1} \sim p_0^{h+1}} p_0^h(\theta^{h} \in \Omega^h(\theta^{h+1},\epsilon))^{-\alpha/(1-\alpha)} < \infty .
\]
\end{definition}

We will prove the following theorem, which generalize Theorem~\ref{thm:regret}.
\begin{theorem}
When $\eta b^2 \leq 1$, we have
\begin{align*}
   & \sum_{t=1}^T 
    \rE_{S_{t-1},x_{t}^1} \rE_{\theta_t \sim \hat{p}_t}  R(\theta_t,x_t^1)\\
    \leq &
    \frac{\lambda}{\alpha \eta} \dc(\Omega,T,0.25\alpha\eta/\lambda)
+ (T/\lambda) \sum_{h=1}^H [\kappa^h(\alpha,\epsilon) - \ln p_0^h(\Omega^h(\epsilon,\theta_*^{h+1}))]\\
 &+ 
    \frac{\alpha}{\lambda} \epsilon (\epsilon+4\eta \epsilon+2b) T(T-1) H + \lambda T \epsilon .
\end{align*}
\label{thm:regret-general}
\end{theorem}


Let
\begin{align}
\label{eqn:Qdef}
\hat{Q}_t^h(\theta)=& 
- (1-\alpha)  \ln p_0^h(\theta^h)
- \alpha \sum_{s=1}^{t-1}
\eta 
\ln \tilde{p}(\theta^h|\theta^{h+1},S_{t-1}) \\
=& 
- \ln p_0^h(\theta^h)
+ \alpha \eta \sum_{s=1}^{t-1}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s)\nonumber\\
&\qquad - \alpha \ln \rE_{\tilde{\theta}^h \sim p_0^h(\theta^h)}
\exp 
\bigg(-
\sum_{s=1}^{t-1}\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s\bigg)
 ,
\nonumber
\end{align}
where
\begin{align*}
&\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))\\
=& L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))
-\eta \bigg((\bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h) + (\rE \; [r^h|x_s,a_s]
- (r^h + f^{h+1}(\theta^{h+1},x_s^{h+1}) \bigg)^2\\ 
=& \eta \bigg({f}^{h}(\theta^{h},x_s^h,a_s^h) + 
- (r^h + f^{h+1}(\theta^{h+1},x_s^{h+1}) \bigg)^2\\
&-\eta \bigg((\bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h) + \rE \; [r^h|x_s,a_s])
- (r^h + f^{h+1}(\theta^{h+1},x_s^{h+1}) \bigg)^2 .
\end{align*}
Now, with
\[
\Delta f^1(\theta^1,x_t^1)
= f^1(\theta^1,x_t^1)-f^1(\theta_*,x_t^1) ,
\]
we obtain from the definition of $\hat{p}_t$:
\begin{equation}
\hat{p}_t(\theta) \propto \exp\bigg(-\sum_{h=1}^H\hat{Q}_t^h(\theta)+ \lambda \Delta f^1(\theta^1,x_t^1) \bigg) .
\label{eq:expo}
\end{equation}
This implies the following inequality, which is the basis of our analysis. 
\begin{lemma}
\begin{align*}
&\rE_{\theta \sim \hat{p}_t(\theta)}
\bigg(\sum_{h=1}^H \hat{Q}_t^h(\theta) - \lambda \Delta f^1(\theta^1,x_t^1)+ \ln \hat{p}_t(\theta)\bigg)\\
 =& \inf_p \rE_{\theta \sim p(\cdot)} \bigg(\sum_{h=1}^H \hat{Q}_t^h(\theta) - \lambda \Delta f^1(\theta^1,x_t^1)+ \ln p(\theta) \bigg) .
\end{align*}
\label{lem:basic-bound}
\end{lemma}
\begin{proof}
This is a direct consequence of the well-known fact that \eqref{eq:expo} is the minimizer of the right hand side. 
This fact is equivalent to the fact that the KL-divergence of any $p(\cdot)$ and $\hat{p}_t$ is non-negative. 
\end{proof}

We also have the following bound, which is needed to estimate the left hand side and right hand side of Lemma~\ref{lem:basic-bound}. 
\begin{lemma}
For fixed parameters $[\theta^h,\theta^{h+1}]$, we have
\[
\rE_{[x_s^{h+1},r_s^h]|[x_s^h,a_s^h]}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))
= \eta ( \Delta f^h(\theta_t^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta_t^{h+1},x_s^h,a_s^h))^2 .
\]
Moreover, we have
\[
\rE_{[x_s^{h+1},r_s^h]|[x_s^h,a_s^h]}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))^2
\leq \eta^2 b^2 ( \Delta f^h(\theta_t^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta_t^{h+1},x_s^h,a_s^h))^2 .
\]
\label{lem:exp-var}
\end{lemma}
\begin{proof}
We have the following Bellman's equation: 
\begin{equation}
f^h(\theta_*^h,x^h,a^h) - \bar{f}^{h+1}(\theta_*^{h+1},x^h,a^h) = \rE \; [r^{h}|x^h,a^h] .
\label{eq:bellman}
\end{equation}

For notational simplicity, we introduce $Z=f^h(\theta^h,x_s^h,a_s^h)-(r_s^h+f^{h+1}(\theta^{h+1},x_s^{h+1}))$ as a random variable which depends on $[r_s^h, x_s^{h+1}]$,
conditioned on $[x_s^h,a_s^h]$. 
Then 
\[
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))
= Z^2 - (Z - \rE Z)^2 .
\]
Since
\[
\rE [Z^2 - (Z - \rE Z)^2] = (\rE Z)^2 ,
\]
we obtain
\begin{align*}
&\rE_{[x_s^{h+1},r_s^h]|[x_s^h,a_s^h]}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))\\
=& \bigg(f^h(\theta^h,x_s^h,a_s^h)- (\bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h)+\rE \; [r_s^{h}|x_s^h,a_s^h] )\bigg)^2 .
\end{align*}
Now by expressing $\rE \; [r^{h}|x^h,a^h]$ using \eqref{eq:bellman}, we obtain the first desired equation in the lemma.

Also since $Z \in [-b,b-1]$ and $\max Z- \min Z \leq b$, we have
\[
\rE (Z^2 -(Z- \rE Z)^2)^2 =
(\rE Z)^2 [4 \rE Z^2 - 3 (\rE Z)^2] 
\leq b^2 (\rE Z)^2 .
\]
This leads to the second desired inequality.
\end{proof}

The above lemma implies the following exponential moment estimate. 
\begin{lemma}
If $\eta b^2 \leq 1$, then for all $[\theta^h,\theta^{h+1}]$:
\begin{align*}
&\ln \rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} 
\exp (-\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))\\
\leq& 
- 0.25 \eta ( \Delta f^h(\theta_t^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta_t^{h+1},x_s^h,a_s^h))^2 .
\end{align*}
\label{lem:exp-moment}
\end{lemma}
\begin{proof}
From $\eta b^2 \leq 1$, we know that
\[
\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s) \in [-1,1] .
\]
This implies that 
\begin{align*}
&\exp(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s))\\
=& 1 -  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)
+\psi(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s))
\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)^2\\
\leq &
1 -  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)
+ 0.75 \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)^2 ,
\end{align*}
where we have used the fact that
$\psi(z)=(e^z-1-z)/z^2$ is an increasing function of $z$, and $\psi(1) < 0.75$.
It follows from Lemma~\ref{lem:exp-var} that
\begin{align*}
&\ln \rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} \; 
\exp(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)) \\
\leq & 
\rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} 
 \; \exp(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s))- 1\\
\leq&
-  \rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h}  
\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)
+ 0.75 
\rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} 
\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)^2 \\
\leq & -0.25
\eta ( \Delta f^h(\theta_t^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta_t^{h+1},x_s^h,a_s^h))^2 ,
\end{align*}
where the first inequality is due to $\ln z \leq z-1$.
This proves the desired bound.
\end{proof}
The following lemma upper bounds the right hand side of Lemma~\ref{lem:basic-bound}.
\begin{lemma}
If $\eta b^2 \leq 1$, then
\begin{align*}
&\inf_{p} \; \rE_{S_{t-1},x_t}
 \rE_{\theta \sim p(\cdot)} \bigg[\sum_{h=1}^H \hat{Q}_t^h(\theta)
 -\lambda \Delta f^1(\theta^1,x_t^1)+
 \ln p(\theta) \bigg]\\
 \leq& \lambda \epsilon + 4\alpha \eta (t-1) H \epsilon^2 
 - \sum_{h=1}^H \ln p_0^h(\Omega^h(\epsilon,\theta_*^{h+1})) .
\end{align*}
\label{lem:basic-upper-bound}
\end{lemma}
\begin{proof}
Consider $[\tilde{\theta}^h,\theta^{h+1}]$ that only depends on $S_{s-1}$. Then
from the proof of Lemma~\ref{lem:exp-moment},
we obtain  
\begin{align}
 &\rE_{x_s,a_s,r_s} \; \exp(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)) - 1\nonumber\\
 \leq& -0.25
 \eta ( \Delta f^h(\tilde{\theta}_t^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta_t^{h+1},x_s^h,a_s^h))^2
\leq 0 . \label{eq:partition}
\end{align}
Now, let
\[
W_t^h = 
\rE_{S_{t}}
 \rE_{\theta \sim p(\cdot)}
 \ln \rE_{\tilde{\theta}^h \sim p_0^h}
\exp\bigg(-  \sum_{s=1}^t \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg) ,
\]
then using the notation
\[
\hat{q}_t^h(\tilde{\theta}^h|\theta^{h+1},S_{t-1})
= 
\frac{
\exp\bigg(-  \sum_{s=1}^{t-1} \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg)}
{\rE_{\tilde{\theta}^h \sim p_0^h}
\exp\bigg(-  \sum_{s=1}^{t-1} \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg)} ,
\]
we have
\begin{align*}
&W_s^h-W_{s-1}^h
=
\rE_{S_{s}}
 \rE_{\theta \sim p(\cdot)}
 \ln 
 \rE_{\tilde{\theta}^h \sim \hat{q}_s^h(\cdot|\theta^{h+1},S_{s-1})}
\exp\bigg(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg)\\
\leq&
\rE_{S_{s-1}}
 \rE_{\theta \sim p(\cdot)}
 \rE_{\tilde{\theta}^h \sim \hat{q}_s^h(\cdot|\theta^{h+1},S_{s-1})}
\rE_{x_s,a_s,r_s}\bigg(
\exp\bigg(-  \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg)-1\bigg)
\leq 0 ,
\end{align*}
where the first inequality is due to $\ln z \leq z-1$, and the second inequality is from \eqref{eq:partition}. 

By noticing that $W_0^h=0$, we obtain
\[
W_t^h= W_0^h + \sum_{s=1}^t [W_s^h-W_{s-1}^h] \leq 0 .
\]
That is, for all $\theta^{h+1}$:
\begin{equation}
\rE_{S_{t-1}}
 \rE_{\theta \sim p(\cdot)}
 \ln \rE_{\tilde{\theta}^h \sim p_0^h}
\exp\bigg(-  \sum_{s=1}^{t-1} \Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg) \leq 0.
\label{eq:rhs-log-expo-moment}
\end{equation}
This implies that for an arbitrary $p(\cdot)$:
\begin{align*}
    &\rE_{S_{t-1},x_t}
 \rE_{\theta \sim p(\cdot)} \bigg[\sum_{h=1}^H \hat{Q}_t^h(\theta) -\lambda \Delta f^1(\theta^1,x_t^1)+ \ln p(\theta) \bigg]\\
 =& 
 \rE_{S_{t-1},x_t}
 \rE_{\theta \sim p(\cdot)} \bigg[-\lambda \Delta f^1(\theta^1,x_t^1)+\alpha \sum_{h=1}^H  
  \sum_{s=1}^{t-1}\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\\
&+ \alpha \sum_{h=1}^H\ln \rE_{\tilde{\theta}^h \sim p_0^h}
\exp\bigg(-  \sum_{s=1}^{t-1}\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s)\bigg) + \ln \frac{p(\theta)}{p_0(\theta)} \bigg] \\
 \leq& 
 \rE_{S_{t-1},x_t}
 \rE_{\theta \sim p(\cdot)} \bigg[-\lambda \Delta f^1(\theta^1,x_t^1)+\sum_{h=1}^H \alpha \eta \sum_{s=1}^{t-1}( \Delta f^h(\theta^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h))^2\\
& + \ln \frac{p(\theta)}{p_0(\theta)} \bigg] ,
\end{align*}
where in the derivation of the inequality, we have used \eqref{eq:rhs-log-expo-moment}, and  we have also used the first equality of Lemma~\ref{lem:exp-var} to bound the expectation of $\Delta L(\cdot)$. 

Note that if for all $h$
\[
\theta^h \in \Omega^h(\epsilon,\theta_*^{h+1}) ,
\]
then $|\Delta f(\theta,x_s^h,a_s^h)| \leq \epsilon$, and therefore 
\[
\sum_{h=1}^H \alpha \eta \sum_{s=1}^{t-1}( \Delta f^h(\theta^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h))^2
\leq 4 H (t-1) \epsilon^2 .
\]
By taking $p(\theta)=p_0(\theta) I(\theta \in \Omega(\epsilon))/p_0(\Omega(\epsilon))$, with $\Omega(\epsilon)=\prod_h \Omega^h(\epsilon,\theta_*^{h+1})$, we obtain the desired bound.
\end{proof}
The following lemma lower bounds the entropy term on the left hand side of Lemma~\ref{lem:basic-bound}.
\begin{lemma}
We have 
\[
\rE_{\theta \sim \hat{p}_t(\theta)}
\ln \hat{p}_t(\theta)
\geq \alpha  \rE_{\theta \sim \hat{p}_t(\theta)}
\ln \hat{p}_t(\theta)
+ (1-\alpha) 
\rE_{\theta \sim \hat{p}_t(\theta)}
\sum_{h=1}^H \ln \hat{p}_t(\theta^h) .
\]
\label{lem:entropy-bound}
\end{lemma}
\begin{proof}
The bound follows from the following inequality
\[
\rE_{\theta \sim \hat{p}_t(\theta)}
\ln \frac{\hat{p}_t(\theta)}
{\prod_{h=1}^H \hat{p}_t(\theta^h)}
\geq 0 ,
\]
which is equivalent to the known fact that mutual information is non-negative (or KL-divergence is non-negative). 
\end{proof}

 
We will use the following decomposition to lower bound the left hand side of Lemma~\ref{lem:basic-bound}.
\begin{lemma}
\begin{align*}
& \rE_{S_{t-1},x_t^1} \; \rE_{\theta \sim \hat{p}_t(\theta)}
\bigg(\sum_{h=1}^H \hat{Q}_t^h(\theta) - \lambda \Delta f^1(\theta^1,x_t^1)+ \ln \hat{p}_t(\theta)\bigg) \\
\geq & 
\underbrace{\rE_{S_{t-1},x_t^1} \; \rE_{\theta \sim \hat{p}_t(\theta)}
\bigg[- \lambda \Delta f^1(\theta^1,x_t^1) 
+ (1-\alpha) \ln \frac{\hat{p}_t(\theta^1)}{p_0^1(\theta^1)}
\bigg]}_{A} \\
& +  \underbrace{\alpha
\rE_{S_{t-1},x_{t}^1}\;
\rE_{\theta \sim \hat{p}_t(\theta)}
\left[\sum_{h=1}^H
\sum_{s=1}^{t-1} \Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s) 
+  \ln \frac{\hat{p}_t(\theta)}{\prod_{h=1}^H p_0^h(\theta^h)}
\right]}_{B}
\\
& + 
\sum_{h=1}^H
\underbrace{\rE_{S_{t-1},x_t^1}\; 
\rE_{\theta \sim \hat{p}_t(\theta)}
\left[\alpha 
\ln \rE_{\tilde{\theta}^h \sim p_0^h}
\exp \left(\sum_{s=1}^{t-1} -\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s) \right) + (1-\alpha) \ln \frac{\hat{p}_t(\theta^{h+1})}{p_0^{h+1}(\theta^{h+1})}
\right]}_{C_h}
.
\end{align*}
\label{lem:decomp}
\end{lemma}
\begin{proof}
We note that
\begin{align*}
\hat{Q}_t^h(\theta)
=& -  \ln p_0^h(\theta^h)
+ \alpha \sum_{s=1}^{t-1}  \Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s))\\
&+ \alpha \ln \rE_{\theta^h \sim p_0^h}
\exp \left(-\sum_{s=1}^{t-1} \Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)\right) .
\end{align*}
Now we can simply apply Lemma~\ref{lem:entropy-bound}. 
\end{proof}
We have the following result for $A$ in Lemma \ref{lem:decomp}, with prior of \eqref{eq:conditional-posterior-comp}. Similar results can be obtained with prior of \eqref{eq:conditional-posterior-comp-2}.
\begin{lemma}
We have
\[
A
\geq - \lambda \rE_{S_{t-1},x_t^1}\; \rE_{\theta_t \sim \hat{p}_t(\cdot)}
 \Delta f^1(\theta_t^1,x_t^1) .
\]
\label{lem:A}
\end{lemma}
\begin{proof}
This follows from the fact that
the following KL-divergence is nonnegative:
\[
\rE_{\theta_t \sim \hat{p}_t(\cdot)}
  \ln \frac{\hat{p}_t(\theta_t^1)}{p_0^1(\theta_t^1)}
\geq 0 .
\]
\end{proof}

The following proposition is from \cite{zhang2005data} . The proof is included for completeness.
\begin{proposition}
For each fixed $\theta$, and $s$ and $h$, we define a random variable
\begin{align*}
\xi_s^h(x_s^{h+1},r_s^h,x_s^h,a_s^h)
=&
- \Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)\\
&-
\ln \rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} 
\exp (-\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)) .
\end{align*}
Then 
\[
\rE_{S_{t-1}}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^H 
\xi_s^h(x_s^{h+1},r_s^h,x_s^h,a_s^h)
\bigg)
= 1 .
\]
\label{prop:martingale}
\end{proposition}
\begin{proof}
We can prove the proposition by induction. Assume that the equation 
\[
\rE_{S_{t-1}}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^{H} 
\xi_s^h(x_s^{h+1},r_s^h,x_s^h,a_s^h)
+ \sum_{h=1}^{\tilde{h}-1}
\xi_t^h(x_t^{h+1},r_t^h,x_t^h,a_s^h)
\bigg)
= 1 
\]
for some $t$ and $1 \leq \tilde{h} \leq H$.
Then 
\begin{align*}
&\rE_{S_{t}}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^{H} 
\xi_s^h(x_s^{h+1},r_s^h,x_s^h,a_s^h)
+ \sum_{h=1}^{\tilde{h}}
\xi_t^h(x_t^{h+1},r_t^h,x_t^h,a_s^h)
\bigg)\\
=& 
\rE_{S_{t}}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^{H} 
\xi_s^h(x_s^{h+1},r_s^h,x_s^h,a_s^h)
+ \sum_{h=1}^{\tilde{h}-1}
\xi_t^h(x_t^{h+1},r_t^h,x_t^h,a_s^h)
\bigg)\\
&\cdot \rE_{[x_{s}^{\tilde{h}+1},r_s^{\tilde{h}}]|x_s^{\tilde{h}},a_s^{\tilde{h}}}
\exp 
\bigg(\xi_t^{\tilde{h}}(x_t^{\tilde{h}+1},r_t^{\tilde{h}},x_t^{\tilde{h}},a_t^{\tilde{h}})\bigg)\\
=& 
\rE_{S_{t}}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^{H} 
\xi_s^h(x_s^{h+1},r_s^h,x_s^h,a_s^h)
+ \sum_{h=1}^{\tilde{h}-1}
\xi_t^h(x_t^{h+1},r_t^h,x_t^h,a_s^h)
\bigg) = 1. 
\end{align*}
Note that in the derivation, we have used the fact that
\[
\rE_{[x_{s}^{\tilde{h}+1},r_s^{\tilde{h}}]|x_s^{\tilde{h}},a_s^{\tilde{h}}}
\exp 
\bigg(\xi_t^{\tilde{h}}(x_t^{\tilde{h}+1},r_t^{\tilde{h}},x_t^{\tilde{h}},a_t^{\tilde{h}})\bigg)  = 1.
\]
The desired result now follows from induction. 
\end{proof}
The following lemma bounds $B$ in Lemma~\ref{lem:decomp}.
This is a key estimate in our analysis. 
\begin{lemma}
Assume $\eta b^2 \leq 1$.
Then 
\begin{align*}
 B
\geq & 
0.25\eta \sum_{s=1}^{t-1} \sum_{h=1}^H
\rE_{S_{t-1},x_t^1}\;
 \rE_{\theta_t \sim \hat{p}_t}
 ( \Delta f^h(\theta_t^h,x_s^h,a_s^h)
- \Delta \bar{f}^{h+1}(\theta_t^{h+1},x_s^h,a_s^h))^2 .
\end{align*}
\label{lem:B}
\end{lemma}
\begin{proof}
Given any fixed $\theta$, we can
define a random variable
\[
\xi_s^h(\theta)
= - \Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)
-
\ln \rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} 
\exp (-\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)) 
\]
which depends on $x_s,a_s,r_s$.

It follows that
\begin{align*}
 &  \rE_{\theta \sim \hat{p}_t(\theta)} \left[\sum_{s=1}^{t-1}
    \sum_{h=1}^H -\xi_s^h(\theta) +
    \ln \frac{\hat{p}_t(\theta)}{\prod_{h=1}^H p_0^h(\theta^h)}
\right]
\geq \inf_p \rE_{\theta \sim p()}
\left[\sum_{s=1}^{t-1}
    \sum_{h=1}^H -\xi_s^h(\theta) +
    \ln \frac{p(\theta)}{\prod_{h=1}^H p_0^h(\theta^h)}\right]\\
=& - \ln 
\rE_{\theta \sim \prod_{h=1}^H p_0^h(\theta^h)}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^H \xi_s^h(\theta)\bigg) ,
\end{align*}
where the minimum over $p$ is achieved at
\[
p(\theta) \propto 
\prod_{h=1}^H p_0^h(\theta^h)
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^H \xi_s^h(\theta)\bigg) .
\]
 This implies that
\begin{align*}
 &  \rE_{S_t}\rE_{\theta \sim \hat{p}_t(\theta)} \left[\sum_{s=1}^{t-1}
    \sum_{h=1}^H -\xi_s^h(\theta) +
    \ln \frac{\hat{p}_t(\theta)}{\prod_{h=1}^H p_0^h(\theta^h)}
\right]\\
\geq&
-\rE_{S_t}
\ln 
\rE_{\theta \sim \prod_{h=1}^H p_0^h(\theta^h)}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^H \xi_s^h(\theta)\bigg) \\
\geq&
- \ln 
\rE_{\theta \sim \prod_{h=1}^H p_0^h(\theta^h)} \;
\rE_{S_t}
\exp\bigg(\sum_{s=1}^{t-1}\sum_{h=1}^H \xi_s^h(\theta)\bigg) = 0 .
\end{align*}
The derivation used the concavity of $\log$ and 
Proposition~\ref{prop:martingale}. 
We can now use Lemma~\ref{lem:exp-moment} to bound
\[
\ln \rE_{[x_{s}^{h+1},r_s^h]|x_s^h,a_s^h} 
\exp (-\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)) 
\]
in the definition of $\xi_s^h(\theta)$,
which implies the desired bound. 
\end{proof}    


The following lemma bounds $C_h$ in Lemma~\ref{lem:decomp}.
\begin{lemma}
We have
for all $h \geq 1$:
\begin{align*}
 C_h 
\geq &   
- (1-\alpha)]\rE_{S_{t-1}}
\ln \rE_{\theta^{h+1} \sim p_0^{h+1}}
\bigg(\rE_{\theta^h \sim p_0^h }
\exp\bigg(- \sum_{s=1}^{t-1}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)
\bigg)\bigg)^{-\alpha/(1-\alpha)}
\end{align*}
\end{lemma}     
\begin{proof}
We have
\begin{align*}
&\rE_{\theta \sim \hat{p}_t(\theta)}
\left[\alpha 
\ln \rE_{\tilde{\theta}^h \sim p_0^h}
\exp \left(\sum_{s=1}^{t-1} -\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s) \right) + (1-\alpha) \ln \frac{\hat{p}_t(\theta^{h+1})}{p_0^{h+1}(\theta^{h+1})}
\right]\\
\geq & (1-\alpha)
\inf_{p^{h+1}}
\rE_{\theta \sim p^{h+1}()}
\left[\frac{\alpha}{1-\alpha}
\ln \rE_{\tilde{\theta}^h \sim p_0^h}
\exp \left(\sum_{s=1}^{t-1} -\Delta L^h([\tilde{\theta}^h,\theta^{h+1}],x_s,a_s,r_s) \right) + \ln \frac{p^{h+1}(\theta^{h+1})}{p_0^{h+1}(\theta^{h+1})}
\right]\\
=&  
- (1-\alpha)]
\ln \rE_{\theta^{h+1} \sim p_0^{h+1}()}
\bigg(\rE_{\theta^h \sim p_0^h }
\exp\bigg(- \sum_{s=1}^{t-1}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)
\bigg)\bigg)^{-\alpha/(1-\alpha)} ,
\end{align*}
where the inf over $p^{h+1}$ is achieved at
\[
p^{h+1}(\theta^{h+1})
\propto p_0^{h+1}(\theta^{h+1})
\bigg(\rE_{\theta^h \sim p_0^h }
\exp\bigg(- \sum_{s=1}^{t-1}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)
\bigg)\bigg)^{-\alpha/(1-\alpha)} .
\]
This leads to the lemma.
\end{proof}

The above bound implies the following estimate of $C_h$ in Lemma~\ref{lem:decomp}, which is easier to interpret. 
\begin{lemma}
For all $h \geq 1$,  
\[
C_h \geq - \alpha \epsilon (2b+\epsilon) (t-1)
 -  \kappa^h(\alpha,\epsilon) .
\]
\label{lem:C}
\end{lemma}
\begin{proof}
For $\theta^h \in \Omega^h(\epsilon,\theta^{h+1})$,
we have
\begin{align*}
    |\Delta L([\theta^h,\theta^{h+1}],x_s,a_s,r_s)|
    \leq&
    (\Delta f^h(\theta^h,x_s^h,a_s^h)
    -\Delta \bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h)^2\\
   & + 2 b
    |\Delta f^h(\theta^h,x_s^h,a_s^h)
    -\Delta \bar{f}^{h+1}(\theta^{h+1},x_s^h,a_s^h|\\
    \leq& \epsilon (2b+\epsilon) .
\end{align*}
It follows that
\[
\rE_{\theta^h \sim p_0^h }
\exp\bigg(- \sum_{s=1}^{t-1}
\Delta L^h([\theta^h,\theta^{h+1}],x_s,a_s,r_s)
\bigg) 
\leq p_0^h(\Omega^h(\epsilon,\theta^{h+1}))
\exp(- (t-1) (2b+\epsilon)\epsilon) .
\]
This implies the bound.
\end{proof}

The following result, referred to as the value-function error decomposition in \cite{jiang2017contextual}, is well-known. 
\begin{proposition}
 Given any $\theta_t$, $x_t^0$. Let $[x_t,a_t,r_t]\sim p(\cdot|\theta_t,x_t^0)$ be the trajectory of the greedy policy $\pi(\theta_t)$, we have
  \begin{align*}
  R(\theta_t)
   =&
  \rE_{[x_t,a_t,r_t]\sim p(\cdot|\theta_t)}
 \sum_{h=1}^H  [\Delta f^h(\theta_t,x_t^h,a_t^h)-\Delta \bar{f}^{h+1}(\theta_t,x_t^h,a_t^h)]
  - \rE_{x_t^1} \Delta f^1(\theta_t,x_t^1) .
  \end{align*}
  \label{prop:value-decomposition}
\end{proposition}

We are now ready to prove Theorem~\ref{thm:regret-general}. 
Let
\[
\delta_t^h =\lambda [\Delta f^h(\theta_t,x_t^h,a_t^h)-\Delta \bar{f}^{h+1}(\theta_t,x_t^h,a_t^h)]
- 0.25 \alpha \eta \sum_{s=1}^{t-1}
[\Delta f^h(\theta_t,x_s^h,a_s^h)-\Delta \bar{f}^{h+1}(\theta_t,x_s^h,a_s^h)]^2 .
\]
Then from the definition of decoupling coefficient, we obtain
\begin{equation}
\sum_{t=1}^T
\rE_{S_{t-1},x_t^1}
 \rE_{\theta_t \sim \hat{p}_t}
 \rE_{[x_t,a_t,r_t]\sim p(\cdot|\theta_t,x_t^1)}
 \sum_{h=1}^H \delta_t^h 
\leq 
\frac{\lambda^2}{\alpha \eta} \dc(\Omega,T,0.25\alpha\eta/\lambda) .
\label{eq:delta-dc}
\end{equation}

From Proposition~\ref{prop:value-decomposition}, we obtain
\begin{align*}
&    \rE_{S_{t-1},x_{t}^1} \rE_{\theta_t \sim \hat{p}_t} \lambda R(\theta_t,x_t^1)
 - \rE_{S_{t-1},x_t^1}
 \rE_{\theta_t \sim \hat{p}_t}
 \rE_{[x_t,a_t,r_t]\sim p(\cdot|\theta_t,x_t^1)}
 \sum_{h=1}^H \delta_t^h  \\
=& - \lambda \rE_{S_{t-1},x_{t}^1} \rE_{\theta_t \sim \hat{p}_t}
\rE_{x_t^1} \Delta f^1(\theta_t,x_t^1)\\ 
&+ 0.25 \alpha \eta \sum_{h=1}^H  \sum_{s=1}^{t-1}
\rE_{S_{t-1},x_{t}^1} 
\rE_{\theta_t \sim \hat{p}_t}
\bigg(\Delta f^h(\theta_t,x_s^h,a_s^h)-\Delta \bar{f}^{h+1}(\theta_t,x_s^h,a_s^h)\bigg)^2 \\
\leq& 
\rE_{S_{t-1},x_t^1} \; \rE_{\theta \sim \hat{p}_t(\theta)}
\bigg(\sum_{h=1}^H \hat{Q}_t^h(\theta) - \lambda \Delta f^1(\theta^1,x_t^1)+ \ln \hat{p}_t(\theta)\bigg)\\
&+ \alpha \epsilon(2b+\epsilon) (t-1) H
 + \sum_{h=1}^H \kappa^h(\alpha,\epsilon)\\
 =&\rE_{S_{t-1},x_t^1} \; \inf_{p} \rE_{\theta \sim p(\theta)}
\bigg(\sum_{h=1}^H \hat{Q}_t^h(\theta) - \lambda \Delta f^1(\theta^1,x_t^1)+ \ln \hat{p}_t(\theta)\bigg)\\
&+ \alpha \epsilon(2b+\epsilon) (t-1) H
 + \sum_{h=1}^H \kappa^h(\alpha,\epsilon)\\
 \leq& \lambda \epsilon
  + \alpha \epsilon(\epsilon+4\eta \epsilon+2b) (t-1) H
 - \sum_{h=1}^H \ln p_0^h(\Omega^h(\epsilon,\theta_*^{h+1}))
 +\sum_{h=1}^H \kappa^h(\alpha,\epsilon) .
\end{align*}
The first equality used the definition of $\delta_t^h$.
The first inequality used Lemma~\ref{lem:decomp} and Lemma~\ref{lem:A} and Lemma~\ref{lem:B} and Lemma~\ref{lem:C}.
The second equality used Lemma~\ref{lem:basic-bound}. The second inequality follows from Lemma~\ref{lem:basic-upper-bound}. 

By summing over $t=1$ to $t=T$, and use \eqref{eq:delta-dc}, we obtain the desired bound.

\section{Estimating Decoupling Coefficient}
We require the following Lemma to prove the reduction of Bellman-Eluder dimension to the decoupling coefficient.

\begin{lemma}
Let $\mu_1,\mu_2,\dots\mu_{t-1}$ denote the measures over $S\times A$ obtained by following the policy induced by $(\theta_s)_{s=1}^{t-1}$ at stage $h$ and $\{\nu_1,\dots,\nu_M\}$ be the set of unique measures in this set in decreasing order of occurrences and let $(N_i)_{i=1}^M$ be the number of times a measure appears in the sequence.
If the the Belmman-Eluder Dimension is $E$, then 
\begin{align*}
    &\sum_{s=1}^{t-1}\rE_{x,a\sim\mu_s}(
\Delta f^h(\theta_t^h,x,a) -
\Delta \bar{f}^{h+1}(\theta_t^h,x,a) )^2 \\
&\qquad\qquad\geq w_t^h(\rE_{x,a\sim\mu_t}[
\Delta f^h(\theta_t^h,x,a) -
\Delta \bar{f}^{h+1}(\theta_t^h,x,a) ])^2\\
&\mbox{where }w_t=\begin{cases}N_i &\mbox{ if }\mu_t=\nu_i \land i\in[E-1]\\
\lceil\frac{\sum_{i=E}^MN_i}{E}\rceil&\mbox{ otherwise.} 
\end{cases}
\end{align*}
\end{lemma}
\begin{proof}

If $\mu_t=\nu_i$, then the statement follows from Jensen's inequality.
Otherwise by by the Bellman-Eluder dimension, for any set  $(\mu'_i)_{i=1}^E$  of pairwise different measures, it holds that
\begin{align*}
    \sum_{i=1}^E \rE_{x,a\sim\mu'_i}(
\Delta f^h(\theta_t^h,x,a) -
\Delta \bar{f}^{h+1}(\theta_t^h,x,a))^2 
&\geq (\rE_{x,a\sim\mu_t}[
\Delta f^h(\theta_t^h,x,a) -
\Delta \bar{f}^{h+1}(\theta_t^h,x,a) ])^2\,. 
\end{align*}
It remains to show that we can construct at least $\lceil\frac{\sum_{i=E}^MN_i}{E}\rceil$ sets of $E$ pairwise different measures.
This follows trivially by selecting sets greedily from the largest remaining duplicates of measures.
\end{proof}
\begin{proof}[Proof of Proposition~\ref{prop:bellman eluder to dc}]
Denote $\epsilon^h_{t,s}=\rE_{[x_s^h,a_s^h]}
[\Delta f^h(\theta_t,x_s,a_s)-\Delta \bar{f}^{h+1}(\theta_*,x_s^h,a_s^h)]$, the LHS is
\begin{align*}
    \sum_{t=1}^{T} \sum_{h=1}^H\epsilon^h_{tt}\leq EH+\epsilon TH+\sum_{t=E+1}^{T} \sum_{h=1}^H\epsilon^h_{tt}\rI\{\epsilon^h_{tt}>\epsilon\}\,.
\end{align*}

On the RHS by Cauchy-Schwarz for any $h\in[H]$:
\begin{align*}
    \mu \sum_{t=1}^T \sum_{s=1}^{t-1} 
{\epsilon^h_{ts}}^2
+ \frac{2E(1+\ln(T))}{4\mu} &\geq \sqrt{(1+\ln(T))\sum_{t=E+1}^Tw_t^h{\epsilon^h_{tt}}^2\rI\{\epsilon^h_{tt}>\epsilon\} }\\
&\geq \sqrt{\frac{E(1+\ln(T))}{\sum_{t=1}^T\frac{1}{w^h_t}}}\sum_{t=1}^T\sum_{t=E+1}^T{\epsilon^h_{tt}}\rI\{\epsilon^h_{tt}>\epsilon\}\,.
\end{align*}
Finally we need to bound 
\begin{align*}
    \sum_{t=1}^T\frac{1}{w_{t}^h}\,.
\end{align*}
Every time the measure $\mu_t$ is in the set of the $E-1$ most common measures, one of the counts $N_i$ for $i\in[E-1]$ increases. Otherwise the count $\sum_{i\geq E}N_i$ increases by 1. Hence
\begin{align*}
    \sum_{t=1}^T\frac{1}{w_t^h}\leq \sum_{i=1}^{E-1}\sum_{t=1}^T\frac{1}{t} + \sum_{t=1}^T\frac{E}{t} \leq 2E(1+\ln(T))\,.
\end{align*}
\end{proof}

\begin{proposition}
Under the linear MDP assumption
\begin{align*}
    \BE_h(f; x^h,a^h)]=\,w^h(f)^T\phi(x^h,a^h),
\end{align*}
where we assume that $\sup_{f\in\cF}||w^h(f)||^2\leq C_1$,$\sup_{x,a\in\cX\times\cA}||\phi(x^h,a^h)||^2\leq C_2$,
we have bounded decoupling coefficient.
\end{proposition}
\begin{proof}
Denote $\phi\ics{s}{h}=\rE_{\pi_{f_s}}[\phi(x^h,a^h)]$ and $\Phi^h_{t}=\lambda I+\sum_{s=1}^{t}\phi(x^h,a^h)\phi(x^h,a^h)^\top$.
\begin{align*}
&
\rE_{\pi_{f_t}}
[ \BE_h(f\ics{t}{}; x_t^h,a_t^h)]
%\Delta f^h(\theta_t,x_t^h,a_t^h) -
%\Delta \bar{f}^{h+1}(\theta_t,x_t^h,a_t^h) ]\\
 -\mu \sum_{s=1}^{t-1} 
\rE_{\pi_{f_s}}
[ \BE_h(f\ics{t}{}; x\ics{s}{h},a\ics{s}{h})^2]
%(\Delta f^h(\theta_t,x_s,a_s)-\Delta \bar{f}^{h+1}(\theta_t,x_s^h,a_s^h))^2
\\
&=
w^h(f\ics{t}{})^\top\phi\ics{t}{h}
 -\mu w^h(f\ics{t}{})^\top\sum_{s=1}^{t-1} 
\rE_{\pi_{f_s}}[\phi(x^h,a^h)\phi(x^h,a^h)^\top]w^h(f\ics{t}{})\\
&\leq 
w^h(f\ics{t}{})^\top\phi\ics{t}{h}
 -\mu w^h(f\ics{t}{})^\top\Phi^h_{t-1}w^h(f\ics{t}{})+\mu\lambda C_1\\
&\leq \frac{1}{4\mu}
(\phi\ics{t}{h})^\top(\Phi_{t-1}^h)^{-1}\phi\ics{t}{h}+\mu\lambda C_1\,,
\end{align*}
where the first inequality uses Jensen's inequality and the second is GM-AM inequality.
Summing over all terms yields
\begin{align*}
    &
    \sum_{t=1}^T\sum_{h=1}^H\bigg[
\rE_{\pi_{f_t}}
[ \BE_h(f\ics{t}{}; x_t^h,a_t^h)]
%\Delta f^h(\theta_t,x_t^h,a_t^h) -
%\Delta \bar{f}^{h+1}(\theta_t,x_t^h,a_t^h) ]\\
 -\mu \sum_{s=1}^{t-1} 
\rE_{\pi_{f_s}}
[ \BE_h(f\ics{t}{}; x\ics{s}{h},a\ics{s}{h})^2]
\bigg]
%(\Delta f^h(\theta_t,x_s,a_s)-\Delta \bar{f}^{h+1}(\theta_t,x_s^h,a_s^h))^2
\\
&\leq \sum_{h=1}^H\bigg[\frac{\ln(\det(\Phi_{T}^h))-d\ln(\lambda)}{4\mu}+\lambda \mu C_1T\bigg]\\
&\leq H(\frac{d\ln(\lambda+TC_2/d)-d\ln(\lambda)}{4\mu} +\lambda\mu C_1T)\,.
\end{align*}
Setting $\lambda=\frac{d}{4\mu^2C_1T}$ finishes the proof.
\end{proof}

==> checklist.tex <==

\section*{Checklist}

\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Algorithm~\ref{alg:ts-rl} is a model free posterior sampling method as claimed and the regret is formalized in Theorem~\ref{thm:regret-general}.}
  \item Did you describe the limitations of your work?
    \answerYes{We state the assumptions required for all results in section~\ref{sec:setting}.We further discuss the computational limitations of our algorithm at the end of section~\ref{sec:algorithm}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This paper is theoretical in nature and we do not foresee any immediate societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{For complete proofs we refer the reader to the appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

